Quantifying Privacy Risks of Masked Language Models Using Membership Inference Attacks

The wide adoption and application of Masked language models~(MLMs) on sensitive data (from legal to medical) necessitates a thorough quantitative investigation into their privacy vulnerabilities -- to what extent do MLMs leak information about their training data? Prior attempts at measuring leakage of MLMs via membership inference attacks have been inconclusive, implying the potential robustness of MLMs to privacy attacks. In this work, we posit that prior attempts were inconclusive because they based their attack solely on the MLM's model score. We devise a stronger membership inference attack based on likelihood ratio hypothesis testing that involves an additional reference MLM to more accurately quantify the privacy risks of memorization in MLMs. We show that masked language models are extremely susceptible to likelihood ratio membership inference attacks: Our empirical results, on models trained on medical notes, show that our attack improves the AUC of prior membership inference attacks from 0.66 to an alarmingly high 0.90 level, with a significant improvement in the low-error region: at 1% false positive rate, our attack is 51X more powerful than prior work.

==> tables/name_cond_thresh.tex <==
  \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}llSSSSSSSSSSSSSS@{}}
	\toprule
	%
	 &{\multirow{2}{*}{Method}}  &\multicolumn{4}{c}{w/o Threshold}	&   {}& \multicolumn{4}{c}{w/ Threshold} \\
	\cmidrule{3-6} \cmidrule{8-11}  
	&   &                               {\#Full Name\&Cond.} &  {Precision}& {\#Name\&Cond.} &  {Precision}    & &    {\#Full Name\&Cond.} &  {Precision}& {\#Name\&Cond.} &  {Precision}   \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
     \multirow{3}{*}{\STAB{Name}} 
      &{~\citeauthor{lehman-etal-2021-bert} (len 100)}&  10	&100.0	&96	    &81.3	    &  &7	    & 100.0&	73  &	86.3            \\
      &\textbf{Gibbs  Sampler (len 20)}&  265&	88.7	&454    &	85.9    &	&207    &	92.8	&341    &	89.4    \\
      &\textbf{MH Sampler (len 20}     &  290&	80.0	&567    &	77.8    &	&226    &	84.5	&409    &	80.9    \\
    \midrule[0.1pt]
	\multirow{3}{*}{\STAB{Regul}} 
    & {~\citeauthor{lehman-etal-2021-bert} (len 100)}  &   0	&0.0&	1157    &64.1   &    &	0   &	0.0 &	724 &	72.8    \\
    & \textbf{Gibbs  Sampler (len 20)}  &   0	&0.0&	438	    &48.2  & 	 &  0   &	0.0 &	324 &	51.2    \\
    & \textbf{MH Sampler (len 20}       &   0	&0.0&	949	    &34.5  & 	 &  0   &	0.0 &	748 &	37.7    \\
	\bottomrule
\end{tabular}


%acc is 0.7107142857142857

==> tables/overview-1b.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
%\begin{tabular}{@{}clSSSSScSSSSS@{}}

\begin{tabular}{@{}cllllllcSSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{2}{c}{{Sample-level}}&{}& \multicolumn{2}{c}{{Patient-level}}   \\
	\cmidrule{3-4} \cmidrule{6-7}
	&  Target model &  {Base}  &{Base-b}& {} & {Base} & {Base-b}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
&(A) Model loss     &  0.662	&0.561&	&0.915	&0.632	\\
&(B) Ours	        &  0.900	&0.960&	&0.992	&0.997 \\
%%%%%%%%%%&&&&&&&\\&&&&&&&&\&\&&&&&&      & & & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Prec.}}
&(A) w/ $\mu$ thresh.   & 61.5	&52.8	&&88.2    &	59.7 \\
&(A) w/ Pop. thresh.    & 61.5	&49.3	&&62.3    &	59.2 \\ 
&(B)  w/ Pop. thresh.   & 99.0	&99.5	&&81.8    &	86.1 \\
%%%%%%%%%%%&&&&&&&\\&&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Rec.}}
&(A) w/ $\mu$ thresh.	& 54.8  &	52.3    &&	45.5	&43.4 \\
&(A) w/ Pop. thresh.    & 37.9  &	20.6    &&	100.0&	90.9\\
&(B)  w/ Pop. thresh.   & 50.9  &	68.8    &&	100.0&	100.0  \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}


==> tables/overview-tab.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
%\begin{tabular}{@{}clSSSSScSSSSS@{}}
\begin{tabular}{@{}clcccccSSSS@{}}

	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{2}{c}{{Sample-level}}&{}& \multicolumn{2}{c}{{Patient-level}}   \\
	\cmidrule{3-4} \cmidrule{6-7}
	&  Non-members &  {MIMIC}  &{i2b2}& {} & {MIMIC} & {i2b2}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
    & (A) Model loss    & 0.662  &	0.812&&	0.915&	1.00	\\
    & (B) Ours	        & 0.900  &	0.881&&	0.992&	1.00  \\
    %%%%%%%%%%&&&&&&&\\&&&&      &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Prec.}}
    & (A) w/ $\mu$ thresh.	& 61.5  &	77.9    &&	88.2    &	100.0   \\
    & (A) w/ Pop. thresh.   & 61.5  &	80.1    &&	62.3    &	90.0    \\
    &(B)  w/ Pop. thresh.	& 99.0  &	94.7    &&	81.8    &	91.7    \\
    %%%%%%%%%%%&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Rec.}}
    &(A) w/ $\mu$ thresh	&   54.8    &	54.8    &&	45.5	&   45.5     \\
    &(A) w/ Pop. thresh.    &   37.9    &	37.7    &&	100.0	&   100.0    \\
    &(B)  w/ Pop. thresh.	&   50.9    &	50.0    &&	100.0	&   100.0    \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}


==> tables/patient-i2b2.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}

	%
\begin{tabular}{@{}clSSSSScSSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{4}{c}{{Short}}&{}& \multicolumn{4}{c}{{Long}}   \\
	\cmidrule{3-6} \cmidrule{8-11}
	&   &  {Base} & {Long} &  {Large} &{Large++}& {} & {Base} &{Long} & {Large}& {Large++}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
    &Baseline   & 100.0&	100.0&	100.0&	100.0&	&100.0	&100.0	&100.0	&100.0	\\
    &Ours	    & 100.0&	100.0&	100.0&	100.0&	&100.0	&100.0	&100.0	&100.0  \\
    %%%%%%%%%%&&&&&&&\\&&&&      &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{2}{*}{\STAB{Prec.}}
    &Baseline	& 100.0	&100.0&	100.0&	100.0&&	100.0  &	100.0&	100.0 &	100.0   \\
    &Baseline 2 & 94.3	&94.3	&97.1&	97.1	&&90.0 &	89.2	&86.1 &	83.2 \\ 
    &Ours	    & 95.2	&95.2	&93.4&	92.5	&&91.7 &	91.7	&90.0 &	90.8  \\
    %%%%%%%%%%%&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{2}{*}{\STAB{Acc.}}
    &Baseline	&   53.5 &	54.5	&58.6 &	52.5& &  45.5 &	47.5	&49.5&	50.5  \\
    &Baseline 2 &   100.0&	100.0&	100.0 &	100.0&&	100.0 &	100.0&	100.0&	100.0 \\
    &Ours	    &   100.0&	100.0&	100.0 &	100.0&&	100.0 &	100.0&	100.0&	100.0  \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}


==> tables/patient-out.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}

	%
\begin{tabular}{@{}clSSSSScSSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{4}{c}{{Short}}&{}& \multicolumn{4}{c}{{Long}}   \\
	\cmidrule{3-6} \cmidrule{8-11}
	&   &  {Base} & {Long} &  {Large} &{Large++}& {} & {Base} &{Long} & {Large}& {Large++}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
    &Baseline   & 62.8&	60.5&	62.4&	66.8&&	91.5&	90.7&	94.1&	93.9	\\
    &Ours	    & 98.4&	98.8&	98.3&	97.8&&	99.2&	99.3&	99.3&	99.3  \\
    %%%%%%%%%%&&&&&&&\\&&&&      &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{2}{*}{\STAB{Prec.}}
    &Baseline	& 59.6&	59.3&	62.4&	63.4&&	88.2&	83.9&	94.2&	92.6   \\
    &Baseline 2 & 55.9&	55.9&	54.7&	54.7&&	62.3&	60.4&	60.4&	57.6 \\ 
    &Ours	    & 61.5&	61.9&	59.3&	57.9&&	81.8&	81.1&	79.2&	76.7  \\
    %%%%%%%%%%%&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
           \midrule[0.1pt]
    \multirow{2}{*}{\STAB{Acc.}}
    &Baseline	&   53.5 &	54.5	&58.6&	52.5&&  45.5 &	47.5 &	49.5 &	50.5  \\
    &Baseline 2 &   100.0&	100.0&	100.0&	100.0&&	100.0&	100.0&	100.0&	100.0 \\
    &Ours	    &   100.0&	100.0&	100.0&	100.0&&	100.0&	100.0&	100.0&	100.0  \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}


==> tables/reconstrcution.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\textwidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\textwidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\textwidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\textwidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}clSSSSScSSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{Removed\%}} &  \multicolumn{2}{c}{{Base}}&{ }& \multicolumn{2}{c}{{Large++}}  \\
	\cmidrule{3-4} \cmidrule{6-7} 
	&    & {Short} & {Long} &  &{Short} & {Long}    \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    &25\%       & 100.00&	56.94	&&     100.00 & 51.18 \\
    &50\%	    & 53.72 & 17.44	&  &  53.49 & 	19.58 \\
  
	\bottomrule
\end{tabular}


==> tables/reference-nopop.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
%\begin{tabular}{@{}clSSSSScSSSSS@{}}

\begin{tabular}{@{}cllllllclSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{2}{c}{{Base}}&{}& \multicolumn{2}{c}{{Base-b}}   \\
	\cmidrule{3-4} \cmidrule{6-7}
	&  Reference Model &  {pubmed}  &{bert-base}& {} & {pubmed} & {bert-base}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
&(A) Model loss     & 0.662 &	0.662   &&	0.561   &	0.561   	\\
&(B) Ours	        & 0.900 &	0.883   &&	0.960   &	0.811   \\
%%%%%%%%%%&&&&&&&\\&&&&&&&\\&&&&      &  & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Prec.}}
&(A) w/ $\mu$ thresh.&  61.5    &	61.5    &&	53.0    &	53.0 \\
&(A) w/ Pop. thresh. &  61.2    &	61.2    &&	44.1    &	44.1 \\ 
&(B)  w/ Pop. thresh.&  88.9    &	87.8    &&	90.2    &	82.9 \\
%%%%%%%%%%%&&&&&&&\\&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Rec.}}
&(A) w/ $\mu$ thresh.& 55.7&	55.7    &&	54.0	&54.0  \\
&(A) w/ Pop. thresh. & 15.6&	15.6    &&	7.8	    &7.8  \\
&(B)  w/ Pop. thresh.& 79.2&	71.5    &&	91.3	&48.0  \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}

==> tables/reference.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.29\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
%\begin{tabular}{@{}clSSSSScSSSSS@{}}

\begin{tabular}{@{}cllllllclSSSS@{}}
	\toprule
	%
	& {\multirow{2}{*}{}} &  \multicolumn{2}{c}{{Base}}&{}& \multicolumn{2}{c}{{Base-b}}   \\
	\cmidrule{3-4} \cmidrule{6-7}
	&  Reference Model &  {pubmed}  &{bert-base}& {} & {pubmed} & {bert-base}  \\
% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    \multirow{2}{*}{\STAB{AUC.}} 
&(A) Model loss     & 0.578	& 0.578    &   &	0.463    &	0.463	\\
&(B) Ours	        & 0.860	& 0.838    &   &	0.932    &	0.823  \\
%%%%%%%%%%&&&&&&&\\&&&&&&&\\&&&&      &  & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Prec.}}
&(A) w/ $\mu$ thresh.&  55.4 &	55.4    &   &	47.7	&47.7 \\
&(A) w/ Pop. thresh. &  53.9 &	53.9    &   &	39.4	&39.4 \\ 
&(B)  w/ Pop. thresh.&  97.9 &	93.7    &   &	98.6	&87.2 \\
%%%%%%%%%%%&&&&&&&\\&&&&&&&\\&&&&     &  & & &&&&&& &  & & && & &
\midrule[0.1pt]
\multirow{3}{*}{\STAB{Rec.}}
&(A) w/ $\mu$ thresh.& 55.2	&55.2	&&52.2	&52.2  \\
&(A) w/ Pop. thresh. & 31.2	&31.2	&&16.1	&16.1  \\
&(B)  w/ Pop. thresh.& 47.0	&46.6	&&63.3	&51.6  \\
    %%%%%%%%%%%&&&&&&&\\
	\bottomrule
\end{tabular}

==> tables/tab_condition.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.24\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}cRcccccc@{}}
	\toprule
	%
	& {Method} & {Full Cond. Recall} & {Partial Cond. Recall} &{\#Conds.}&{\%Samples w/ Cond}	& {KL-Div} &{Top15-match}  \\

% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    %%%%%
    \multirow{3}{*}{\STAB{Name}} 
    %%%%%%%%%%&&&&&&&\\
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}	    &	1.46	&   25.00	&   122 &	359	&   1.83    &   40.00 \\
    &\textbf{Gibbs  Sampler (len 20)}                       &   2.92	&   25.82	&   634 &	368	&   0.89    &   66.67  	\\
    &\textbf{MH Sampler (len 20}                            &	3.74	&   34.06	&   707 &	428	&   1.13    &   60.00  	\\
    %%%%%%%%%&&&&&&&\\  &
    \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Regul.}}  
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}	    &	4.90    &	36.79   &	4049	&   379  &	1.46    &	46.67	   	\\
    &\textbf{Gibbs Sampler (len 20)}                        &	3.11    &	28.26   &	893	    &   370  &	0.81    &	73.33	   	\\
    &\textbf{MH Sampler (len 20}                            &	4.30    &	34.28   &	1835	&   452  &	0.99    &	60.00	   	\\
    %%%%%%%%%%&&&&&&&\\
	%%%%%%%%%
	\bottomrule
\end{tabular}

==> tables/tab_name.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.23\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}cRcccccc@{}}
	\toprule
	%
	& {Method} & {Full Name Recall} & {First Name Recall} &{Last Name Recall}&{\%Samples w/ Full Name}	& {\%Samples. w/  Name}  \\

% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    %%%%%
    \multirow{3}{*}{\STAB{Name}} 
    %%%%%%%%%%&&&&&&&\\
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}	    &	1.032    &	3.62    &	7.02   & 11.64  &	84.94	  	\\
    &\textbf{Gibbs  Sampler (len 20)}                        &   2.059    &	3.48    &	5.93   & 66.98  &	95.98	  	\\
    &\textbf{MH Sampler (len 20}                            &	3.583    &	4.50    &	8.99   & 57.61  &	93.85	  	\\
    %%%%%%%%%&&&&&&&\\  &
    \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Regul.}}  
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}	    &	0.002    &	0.48    &	3.10   & 0.01    &	68.00	   	\\
    &\textbf{Gibbs Sampler (len 20)}                        &	0.000    &	0.16    &	1.88   & 0.00    &	95.84	   	\\
    &\textbf{MH Sampler (len 20}                            &	0.002    &	0.53    &	2.61   & 0.03    &	88.36	   	\\
    %%%%%%%%%%&&&&&&&\\
	%%%%%%%%%
	\bottomrule
\end{tabular}

==> tables/tab_name_condition.tex <==
 \newcolumntype{L}{>{\RaggedLeft\arraybackslash}p{0.06\linewidth}} 
  \newcolumntype{O}{>{\RaggedLeft\arraybackslash}m{0.07\linewidth}} 
  \newcolumntype{D}{>{\arraybackslash}m{0.15\linewidth}} 
  \newcolumntype{R}{>{\arraybackslash}m{0.24\linewidth}} 
% \begin{tabular}{@{}cDrrrrrcrrrr@{}}
\begin{tabular}{@{}cRcccccc@{}}
	\toprule
	%
	& {Method} & {Full Name+Cond. Match} & {Full Name+Cond Mismatch} &{Partial Name+Cond. Match}&{Partial Name+Cond. Mismatch} \\

% 	&Metric &Original &A4NT	&One-LM	 &One-LM (DB25)	 &One-LM (DB40)	 &Inters.	&Inters. (DB25)	&Inters. (DB40)	&Union \\
	%%%%%%%%%
    \midrule
	%%%%%%%%%
    %%%%%
    \multirow{3}{*}{\STAB{Name}} 
    %%%%%%%%%%&&&&&&&\\
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}    &	10&	0	&    99  &   	18    \\
    &\textbf{Gibbs  Sampler (len 20)}                   &   235	&30	&    561	    &   126    	  	\\
    &\textbf{MH Sampler (len 20}                        &   232	&58	&    572 &   	65      	\\
    %%%%%%%%%&&&&&&&\\  &
    \midrule[0.1pt]
    \multirow{3}{*}{\STAB{Regul.}}  
    &{~\citeauthor{lehman-etal-2021-bert} (len 100)}	    &	0   &	0   &	3634    &	415   	\\
    &\textbf{Gibbs Sampler (len 20)}                        &	0   &	0   &	0       &	241   	\\
    &\textbf{MH Sampler (len 20}                            &	0   &	0   &	1127    &  	622   	\\
    %%%%%%%%%%&&&&&&&\\
	%%%%%%%%%
	\bottomrule
\end{tabular}
